Resilience and Security of Deep Neural Networks Against Intentional and Unintentional Perturbations: Survey and Research Challenges

In order to deploy deep neural networks (DNNs) in high-stakes scenarios, it is imperative that DNNs provide inference robust to external perturbations - both intentional and unintentional. Although the resilience of DNNs to intentional and unintentional perturbations has been widely investigated, a unified vision of these inherently intertwined problem domains is still missing. In this work, we fill this gap by providing a survey of the state of the art and highlighting the similarities of the proposed approaches.We also analyze the research challenges that need to be addressed to deploy resilient and secure DNNs. As there has not been any such survey connecting the resilience of DNNs to intentional and unintentional perturbations, we believe this work can help advance the frontier in both domains by enabling the exchange of ideas between the two communities.

==> tex-files/preamble.tex <==
%%%%%%%%%%%%%%%%% Useful stuff %%%%%%%%%%%%
\newcommand{\eq}[1]{Eq.~\eqref{#1}}
\newcommand{\blue}[1]{\textbf{\color{blue}{#1}}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\bit}{\begin{itemize}}
\newcommand{\eit}{\end{itemize}}
\newcommand{\fig}[1]{\figurename~\ref{#1}}
\usepackage[framemethod=tikz]{mdframed}  %%% Highlight para

\newcommand{\todo}[1]{\textbf{\color{red}[XX #1 XX]}}

% \usepackage[center]{titlesec}
\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
\usepackage{bm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%Boxes Start here%%%%%%%%%%%%%%%%%%%
\usepackage[many]{tcolorbox}
\usepackage{lipsum}

\definecolor{titlebg}{RGB}{100,22,72}
\definecolor{introbg}{RGB}{0,128,128}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% Source: https://tex.stackexchange.com/questions/253220/replicate-a-box-using-fancybox
\newtcolorbox{usecase}[1][]{
  breakable,
  enhanced,
  arc=0pt,
  outer arc=0pt,
  colframe=titlebg,
  colback=titlebg!05,
  overlay unbroken and first={
    \node[
      draw=titlebg,
      fill=titlebg,
      rotate=0,
      anchor=north west,
      text=white,
      font=\bfseries
    ]
    at (frame.north west)  
    {#1};
  }
}

\newtcolorbox{mission}[1][]{
  breakable,
  enhanced,
  arc=0pt,
  outer arc=0pt,
  colframe=introbg,
  colback=introbg!05,
  overlay unbroken and first={
    \node[
      draw=introbg,
      fill=introbg,
      rotate=0,
      anchor=north west,
      text=white,
      font=\bfseries
    ]
    at (frame.north west)  
    {#1};
  }
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
